Radiative neutrino masses in the singlet-doublet fermion dark matter model with scalar singlets

When the singlet-doublet fermion dark matter model is extended with additional $Z_2$--odd real singlet scalars, neutrino masses and mixings can be generated at one-loop level. In this work, we discuss the salient features arising from the combination of the two resulting simplified dark matter models. When the $Z_2$-lightest odd particle is a scalar singlet, $\operatorname{Br}(\mu\to e \gamma)$ could be measurable provided that the singlet-doublet fermion mixing is small enough. In this scenario, also the new decay channels of vector-like fermions into scalars can generate interesting leptonic plus missing transverse energy signals at the LHC. On the other hand, in the case of doublet-like fermion dark matter, scalar coannihilations lead to an increase in the relic density which allow to lower the bound of doublet-like fermion dark matter.

==> details.tex <==
%auto-ignore
%%%%Full definitions
\renewcommand{\DetailsWeylconventions}{
\section{Preliminars}

Check ~\cite{Cheung:2013dua,Dedes:2014hga}

Weyl spinors tranform under Lorentz as shown in Table~\ref{tab:electron}, illustrated for the case of the electron.

\begin{table}
  \centering
  \begin{tabular}{|llll|}
\hline
    Name & Symbol & Lorentz & $U(1)_Q$\\\hline
   $e_L^-$: left electron & $\xi_{\alpha}$ & ${M_{\alpha}}^{\beta}$ & $e^{i\theta}$\\
   $\left( e_L^- \right)^{\dagger}$: right positron    & $\left( \xi_{\alpha} \right)^{\dagger}=\xi^{\dagger}_{\dot{\alpha}}$ & ${{M^{*}}_{\dot{\alpha}}}^{\dot{\beta}}$ & $e^{-i\theta}$\\
   $e_R^-$: right electron   & $\left( \eta^{\alpha} \right)^{\dagger}=\eta^{\dagger\;\dot{\alpha}}$ & ${\left[ \left( M^{-1} \right)^\dagger \right]^{\dot{\alpha}}}_{\dot{\beta}}$& $e^{i\theta}$\\
   $\left( e_R^{-} \right)^{\dagger}$: left positron &$\eta^{\alpha}$& ${\left[ \left( M^{-1} \right)^T \right]^{\alpha}}_{\beta}$ & $e^{-i\theta}$\\\hline
  \end{tabular}
  \caption{Electron components}
  \label{tab:electron}
\end{table}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsWeylspinors}{
\section{Weyl spinors} 

  Consider the following set of Weyl spinors
\begin{align*}
  L=&
      \begin{pmatrix}
  \xi_{1\alpha}\\
  \xi_{2\alpha}
  \end{pmatrix}
  =\begin{pmatrix}
  \nu_L\\
  e_L    
  \end{pmatrix}&
  N=&\eta_1^{\alpha} \nonumber\\
  R_u=&
  \begin{pmatrix}
  \eta_2^{\dagger\dot{\alpha}}\\
  \eta_3^{\dagger\dot{\alpha}}\\
  \end{pmatrix}
  =
  \begin{pmatrix}
   \psi_R^0\\
   \psi_R^-    
  \end{pmatrix}&R_d=&
  \begin{pmatrix}
       \xi_{3\alpha}\\
       \xi_{4\alpha}
  \end{pmatrix}=
  \begin{pmatrix}
      \psi_L^0\\
      \psi_L^-    
  \end{pmatrix}
.\end{align*}
In order to have all the new fields in term of Weyl \emph{left}-fermions, it is convinient to define (the $\dagger$ for Weyl spinors just stands for conjugate)  
\begin{align}
  \widetilde{R}_u= i\sigma_2 R_u^{\dagger}=&i
  \begin{pmatrix}
    0 &-i\\
    i & 0\\
  \end{pmatrix}\begin{pmatrix}
  \eta_2^{\dagger\dot{\alpha}}\\
  \eta_3^{\dagger\dot{\alpha}}\\
  \end{pmatrix}^{\dagger}\nonumber\\
=&
  \begin{pmatrix}
    0 &1\\
    -1 & 0\\
  \end{pmatrix}  \begin{pmatrix}
 \left(   \eta_2^{\dagger\dot{\alpha}} \right)^{\dagger}\\
  \left( \eta_3^{\dagger\dot{\alpha}} \right)^{\dagger}\\
  \end{pmatrix}\nonumber\\
=&\begin{pmatrix}
  \eta_3^{\alpha}\\
  -\eta_2^\alpha\\
  \end{pmatrix}.
 \end{align}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsRddoublet}{
\begin{pmatrix}
R_{d}^0\\    
R_{d}^-
\end{pmatrix}=
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsRudoublet}{
\begin{pmatrix}
 \widetilde{R}_{u}^+\\    
 \widetilde{R}_{u}^0
\end{pmatrix}=
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\Detailscontraction}{
Following the usual convention to contract the index
\begin{align}
  {}_{\alpha}\ {}^{\alpha} \qquad {}^{\dot{\alpha}}\ {}_{\dot{\alpha}}\;,
\end{align}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsInteractionBasis}{
The Lagrangian is
\begin{align}
\label{eq:lt13aib}
  -\mathcal{L}=&M_D \epsilon_{ab}R^a_d \widetilde{R}^b_u+\tfrac{1}{2}M_N NN-h'_{i\alpha} \epsilon_{ab}\widetilde{R}_u^a L_{i}^b S'_{\alpha}-\lambda_d\, \epsilon_{ab}H^a R_d^b N-\lambda_u \epsilon_{ab}\widetilde{H}^a \widetilde{R}_u^b N+\text{h.c}\nonumber\\
&-\left[ \mu^2 \epsilon_{ab}\widetilde{H}^{a}H^b+\tfrac{1}{2}\lambda_1 \left( \epsilon_{ab} \widetilde{H}^{a}H^b\right)^2+\tfrac{1}{2}\left({M'}_S^2\right)_{\alpha\beta} S'_{\alpha}S'_\beta
   +\lambda^{\prime SH}_{\alpha\beta} \epsilon_{ab}\widetilde{H}^{a}H^bS'_{\alpha}S'_{\beta}+\lambda^{\prime S}_{\alpha\beta\gamma\delta}S'_{\alpha}S'_{\beta}S'_{\gamma}S'_{\delta}  \right]
\end{align}
where
\begin{align*}
  {H}=&  \begin{pmatrix}
    H^+ \\ H^0
  \end{pmatrix}&
  \widetilde{H}=&  \begin{pmatrix}
    {H^0}^{*} \\ -H^-
  \end{pmatrix}
\end{align*}
Note that a term like $\epsilon_{ab}\widetilde{R}_d^a L^b$ have the wrong Lorentz sctructure $\xi_{\dot{\alpha}}^{\dagger}\xi_{\alpha}$. 

For the $Z_2$--odd scalars we have in the basis
$
  \mathbf{S}=
  \begin{pmatrix}
    S_1&
    S_2&
    \cdots&
    S_{\alpha}
  \end{pmatrix}^{\operatorname{T}}
$, where now $\alpha,\beta$ is the number of real scalar fields
\begin{align*}
    \mathcal{L}_S=&\frac{1}{2}{\mathbf{S}'}^{\operatorname{T}}{\mathbf{M}'}_S^2\mathbf{S}'
+ \epsilon_{ab}\widetilde{H}^a H^b {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime SH}\mathbf{S}' 
+ S'_{\gamma}\left( {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime S}\mathbf{S}' \right)_{\gamma\delta} S'_{\delta} \nonumber\\
=&\frac{1}{2}{\mathbf{S}'}^{\operatorname{T}}{\mathbf{M}'}_S^2\mathbf{S}'
+ \epsilon_{ab}\widetilde{H}^a H^b {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime SH}\mathbf{S}' 
+ \mathbf{S'}^{\operatorname{T}}\left( {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime S}\mathbf{S}' \right)\mathbf{S'} \,,
\end{align*}


After the spontaneous symmetry breaking
\begin{align}
  \mathcal{L}_S\supset&\frac{1}{2}{\mathbf{S}'}^{\operatorname{T}}{\boldsymbol{\mathcal{M}}'}_S^2\mathbf{S}' \nonumber\\
=&\frac{1}{2}{\mathbf{S}}^{\operatorname{T}}\left( \mathbf{R}^T{\boldsymbol{\mathcal{M}}'}_S^2\mathbf{R} \right)\mathbf{S} \nonumber\\
=&\frac{1}{2}\sum_{\alpha}m^2_{S_{\alpha}}S_{\alpha}^2\,,
\end{align}
where
\begin{align}
  \left( {\mathcal{M}'}_S ^2\right)_{\alpha\beta}
=&\left( {M'}_S^2 \right)_{\alpha\beta}+\lambda^{\prime SH}_{\alpha\beta}v^2\,.
\end{align}
is diagonilized by the ortogonal matriz $\mathbf{R}$. In what follows, we assume a basis in which $\boldsymbol{\mathcal{M}}_S^2$ is already diagonal with
\begin{align*}
 \mathbf{M}_S^2=&\mathbf{R}^{\operatorname{T}} {\mathbf{M}'}_S^2\mathbf{R} \nonumber\\
\boldsymbol{\lambda}^{SH}=&  \mathbf{R}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime SH} \mathbf{R}
\end{align*}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DefineXiInTermsOfR}{
=
\begin{pmatrix}
N & R_d^0 & -\widetilde{R}_u^0   
\end{pmatrix}^{\operatorname{T}}
}
%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsDiracAndMajoranaFermions}{

\section{Dirac and Majorana Fermions}

A fermion is defined to be vector-like if its left- and right-handed chiralities belongs to the same representation of
$SU(3)_C\times SU(2)_L\times U(1)_Y$. For a vector like singlet see \cite{Aoki:2011yk}. We will follow the notation of \cite{Yoshikawa:1995et}.   We now define the corresponding Dirac fermions denoted with a hat. In terms of its Weyl fermions components (without specify the undotted and dotted indices), we have
\begin{align*}
  \widehat{\psi}^-=&
  \begin{pmatrix}
   \psi_{L}^{-}\\
   \psi_{R}^{-}\\
  \end{pmatrix}
&
    \widehat{\psi}^0=&
  \begin{pmatrix}
    \psi_{L}^0\\
    \psi_{R}^0
  \end{pmatrix}
\end{align*}
moreover
\begin{align*}
  \widehat{\psi}_{(L,R)}^-=&P_{L,R}\widehat{\psi}^-&
  \widehat{\psi}_{(L,R)}^0=&P_{L,R}\widehat{\psi}^0
\end{align*}
and Dirac $SU(2)$ doublets
\begin{align*}
  \widehat{\Psi}_{(L,R)}=&P_{L,R}\widehat{\Psi}=P_{L,R}
  \begin{pmatrix}
    \widehat{\psi}^0\\
        \widehat{\psi}^-\\
  \end{pmatrix}=
  \begin{pmatrix}
    \widehat{\psi}^0_{(L,R)}\\
        \widehat{\psi}^-_{(L,R)}\\
  \end{pmatrix},&
  \overline{\widehat{\Psi}_{(L,R)}}=&  \begin{pmatrix}
    \overline{\widehat{\psi}^0}&
        \overline{\widehat{\psi}^-}\\
  \end{pmatrix}P_{R,L}=  \begin{pmatrix}
    \overline{\widehat{\psi}^0_{(L,R)}}&
        \overline{\widehat{\psi}^-_{(L,R)}}\\
  \end{pmatrix}
\end{align*}

Following the notation of \cite{Martin:2012us}
\begin{align*}
  \overline{\widehat{\psi}^-}=\left( {\widehat{\psi}^-} \right)^{\dagger}
  \begin{pmatrix}
    0 & 1\\
   1 & 0
  \end{pmatrix}=&
    \begin{pmatrix}
      \left( \psi_{R}^- \right)^{\dagger} & \left( \psi_{L}^- \right)^{\dagger}
    \end{pmatrix}&
  \overline{\widehat{\psi}^0}=\left( \widehat{\psi}^0 \right)^{\dagger}  \begin{pmatrix}
    0 & 1\\
   1 & 0
  \end{pmatrix}=&\begin{pmatrix}
{\psi_{R}^0 }^{\dagger} & {\psi_{L}^0 }^{\dagger} 
\end{pmatrix}
\end{align*}
Now,we can check the $SU(2)$ mass term
\begin{align}
\label{eq:mdpsipsi}
  \left( \overline{\widehat{\Psi}}_{L}\widehat{\Psi}_{R}+\overline{\widehat{\Psi}}_{R}\widehat{\Psi}_{L} \right)=&  \overline{\widehat{\Psi}}\widehat{\Psi} \nonumber\\
=&   \begin{pmatrix}
    \overline{\widehat{\psi}^0} &  \overline{\widehat{\psi}^-} 
  \end{pmatrix}
  \begin{pmatrix}
    \widehat{\psi}^0 \\
    \widehat{\psi}^-
  \end{pmatrix}\nonumber\\
= & \left(     \overline{\widehat{\psi}^0}\widehat{\psi}^0 +
    \overline{\widehat{\psi}^-} \widehat{\psi}^-
 \right) \nonumber\\
= & \left[
\begin{pmatrix}
{\psi_{R}^0 }^{\dagger} & {\psi_{L}^0 }^{\dagger} 
\end{pmatrix} \begin{pmatrix}
    \psi_{L}^0\\
    \psi_{R}^0
  \end{pmatrix}
+\begin{pmatrix}
      \left(\psi_{R}^{-}\right)^\dagger & \left(\psi_{L}^{-}\right)^\dagger
    \end{pmatrix} \begin{pmatrix}
   \psi_{L}^{-}\\
   \psi_{R}^{-}\\
  \end{pmatrix}
 \right] \nonumber\\
= & \left(
    {\psi_{R}^0 }^{\dagger}\psi_{L}^0+
   {\psi_{L}^0 }^{\dagger} \psi_{R}^0+
   \left(\psi_{R}^{-}\right)^\dagger\psi_{L}^{-}+
   \left(\psi_{L}^{-}\right)^\dagger\psi_{R}^{-}
 \right) \nonumber\\
= & \left(
    {\psi_{R}^0 }^{\dagger}\psi_{L}^0+
    \left(\psi_{R}^{-}\right)^\dagger\psi_{L}^{-}+
 \text{h.c}
 \right)\,.
\end{align}



Then
\begin{align}
\overline{\widehat{\Psi}}\widehat{\Psi} 
=& \left(\widetilde{R}_u^0 R_{d}^0-\widetilde{R}_u^{+}R_d^- +\text{h.c}  \right)  \nonumber\\
=& \left(R_d^1 \widetilde{R}_u^2-R_d^2 \widetilde{R}_u^1 +\text{h.c} \right) \nonumber\\
=& \left(\epsilon_{12}R_d^1 \widetilde{R}_u^2+ \epsilon_{21}R_d^2 \widetilde{R}_u^1 +\text{h.c} \right) \nonumber\\
=& \left(\epsilon_{ab}R_d^a \widetilde{R}_u^b +\text{h.c} \right)\,.
\end{align}

Since
\begin{align*}
  \widehat{e}=&
  \begin{pmatrix}
    e_L\\
    e_R
  \end{pmatrix}&
\widehat{\nu}=&
\begin{pmatrix}
\nu_L\\
0\\  
\end{pmatrix}\nonumber\\
\widehat{e}_L= P_L\widehat{e}=&
  \begin{pmatrix}
    e_L\\
    0
  \end{pmatrix}&
\widehat{\nu}_L=P_L\widehat{\nu}=&
\begin{pmatrix}
\nu_L\\
0\\  
\end{pmatrix}
\end{align*}
\begin{align*}
    \overline{\widehat{e}}=&
  \begin{pmatrix}
  e_R^{\dagger} &   e_L^{\dagger} \\
  \end{pmatrix}&
    \overline{\widehat{\nu}}=&
  \begin{pmatrix}
  0 &   \nu_L^{\dagger} \\
  \end{pmatrix}&
\end{align*}
\begin{align*}
  \widehat{L}=
  \begin{pmatrix}
  \widehat{\nu}_L\\
  \widehat{e}_L    
  \end{pmatrix}
\end{align*}
we have
\begin{align*}
  \epsilon_{ab}\widetilde{R}_{u}^a L^b S +\text{h.c}=
&\left[\widetilde{R}_u^1 L^2- \widetilde{R}_u^2 L^1 \right]S+\text{h.c}\nonumber\\
=&\left[ \widetilde{R}_u^+ e_L -\widetilde{R}_u^0 \nu_L\right]S+\text{h.c}\nonumber\\
=&-\left[ {\psi_{R}^0}^{\dagger}\nu_L  
+\left(\psi_{R}^-\right)^{\dagger} e_L    
 \right]S+\text{h.c} \nonumber\\
=&-\left[   \begin{pmatrix}
  {\psi_{R}^0}^{\dagger} &0\\
\end{pmatrix}
\begin{pmatrix}
\nu_L\\
0
\end{pmatrix}-  \begin{pmatrix}
   \left( \psi_{R}^- \right)^{\dagger} & 0
  \end{pmatrix}
  \begin{pmatrix}
    e_L\\ 
    0
  \end{pmatrix}
 \right]S +\text{h.c}\nonumber\\
=&-\overline{\widehat{\psi}^0}P_L\; P_L\widehat{\nu}S 
+\overline{\widehat{\psi}^-}P_L\;P_L\widehat{e}S
+\text{h.c}\nonumber\\
=&-\overline{\widehat{\psi}_{R}^0}\widehat{\nu}_LS
+\overline{\widehat{\psi}_{R}^-}\widehat{e}_LS
+\text{h.c}\nonumber\\
=&-\overline{\widehat{\Psi}_{R}} {\widehat{L}} S+\text{h.c}\,.
\end{align*}
If we define
\begin{align}
\label{eq:NM}
\widehat{N}=&
\begin{pmatrix}
  N & N^{\dagger}
\end{pmatrix}&
\overline{\widehat{N}}=
\begin{pmatrix}
N & N^{\dagger}   
\end{pmatrix}
\end{align}

\begin{align}
\label{eq:HRdN}
\epsilon_{ab}H^a R_d^b N+\text{h.c}=&H^1 R_d^2 N-H^2 R_d^1 N+\text{h.c}\nonumber\\
 =&H^+ R_d^- N-H^0 R_d^0 N+\text{h.c}\nonumber\\
=&-N H^0 \psi_L^0  +N H^+ \psi_{L}^- +\text{h.c}\nonumber\\
=&- \begin{pmatrix}
   N & 0
 \end{pmatrix}
H^0 
\begin{pmatrix}
  \psi_L^0\\
   0
\end{pmatrix}
+
\begin{pmatrix}
N & 0  
\end{pmatrix}
 H^+ 
  \begin{pmatrix}
\psi_{L}^-\\
   0    
  \end{pmatrix}
+\text{h.c}\nonumber\\
=&-\overline{\widehat{N}}P_L H^0 P_L\widehat{\psi}^0+\overline{\widehat{N}}P_L H^+P_L \widehat{\psi}^-+\text{h.c} \nonumber\\
=&-\overline{\widehat{N}}H^0 P_L\widehat{\psi}^0+\overline{\widehat{N}}H^+P_L \widehat{\psi}^-+\text{h.c} \nonumber\\
=&-\overline{\widehat{N}} H^0 \widehat{\psi}^0_L+\overline{\widehat{N}} H^+\widehat{\psi}^-_L +\text{h.c}\nonumber\\
=&-\overline{\widehat{N}}
\begin{pmatrix}
  H^0 & -H^{+}
\end{pmatrix}
\begin{pmatrix}
\widehat{\psi}_L^0\\
\widehat{\psi}_L^-  
\end{pmatrix}+\text{h.c}\nonumber\\
=&-\overline{\widehat{N}}\widetilde{H}^{\dagger} \widehat{\Psi}_L-\overline{\widehat{\Psi}_L}\widetilde{H} \widehat{N}\,.
\end{align}

Finally
\begin{align}
\label{eq:HRuN}
  \epsilon_{ab}\widetilde{H}^a \widetilde{R}_u^b N+\text{h.c}=&\widetilde{H}^1 \widetilde{R}_u^2 N-\widetilde{H}^2 \widetilde{R}_u^1 N +\text{h.c}\nonumber\\
=&{H^0}^* \widetilde{R}_u^0 N+{H}^-\widetilde{R}_u^+ N +\text{h.c}\nonumber\\
=&-{H^0}^* {\psi_R^0}^{\dagger} N+{H}^- \left( \psi_R^- \right)^{\dagger} N +\text{h.c}\nonumber\\
  =&-\begin{pmatrix}
{\psi_R^0}^{\dagger} & 0    
  \end{pmatrix}{H^0}^*
  \begin{pmatrix}
N\\
0    
  \end{pmatrix}
 +\begin{pmatrix}
\left( \psi_R^- \right)^{\dagger} & 0\\   
 \end{pmatrix}{H}^-
 \begin{pmatrix}
   N\\
   0
 \end{pmatrix}
 +\text{h.c}\nonumber\\
  =&-\overline{\widehat{\psi}^0}P_L{H^0}^* P_L \widehat{N} +
 \overline{\widehat{\psi}^-}P_L{H}^-P_L\widehat{N} +\text{h.c}\nonumber\\
  =&-\overline{\widehat{\psi}^0}P_L{H^0}^* \widehat{N} +
 \overline{\widehat{\psi}^-}P_L{H}^-\widehat{N} +\text{h.c}\nonumber\\
  =&-\overline{\widehat{\psi}^0_R}{H^0}^* \widehat{N} +
 \overline{\widehat{\psi}^-_{R}}{H}^-\widehat{N} +\text{h.c}\nonumber\\
  =&  \begin{pmatrix}
 \overline{\widehat{\psi}^0_R} &  \overline{\widehat{\psi}^-_{R}}
  \end{pmatrix}
  \begin{pmatrix}
{H^0}^*\\
-{H}^-    
  \end{pmatrix}
\widehat{N} +\text{h.c}\nonumber\\
=&-\overline{\widehat{\Psi}_{R}}\widetilde{H}\widehat{N} -\overline{\widehat{N}}\widetilde{H}^{\dagger}\widehat{\Psi}_R\,.
\end{align}


The Full Lagrangian for Dirac and Majorana Fermions is 
\begin{align}
\label{eq:lfull}
  -\mathcal{L}=&M_D \overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}
+h_{i\alpha} \overline{\widehat{\Psi}_{R}} \widehat{L}_i S_{\alpha}
+\lambda_d\overline{\widehat{\Psi}_L}\widetilde{H} \widehat{N}
+\lambda_u\overline{\widehat{\Psi}_{R}}\widetilde{H}\widehat{N}+\text{h.c}\nonumber\\
&-\left[ \mu^2 H^{\dagger}H+\lambda_1 \left(H^{\dagger}H \right)^2+\tfrac{1}{2}\left(M_S^2\right)_{\alpha\beta} S_{\alpha}S_\beta
   +\lambda^{SH}_{\alpha\beta} H^{\dagger}H S_{\alpha}S_{\beta}+\lambda^{S}_{\alpha\beta\gamma\delta}S_{\alpha}S_{\beta}S_{\gamma}S_{\delta} \right]
\end{align}

\section{Alternative notation}
In the Lagrangian implemented in Feynrules the right-handed neutrino have implicitly the proyectors:
\begin{align}
    \mathcal{L}_A=&\left[ h_{i\alpha}\overline{\widehat{L_i}}\widehat{\Psi} S'_{\alpha}+\lambda_d \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H {N}^{c}
+\lambda_u \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H {N}+\text{h.c} \right]
+M_D\overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}
\end{align}
By writing explicitly the projectors we have
\begin{align*}
    \mathcal{L}_A=&\left[ h_{i\alpha}\overline{\widehat{L}}\widehat{\Psi} S'_{\alpha}+\lambda_d \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H P_L\widehat{N}^{c}
+\lambda_u \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H P_R\widehat{N}+\text{h.c} \right]
+M_D\overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}\
\end{align*}
We now focus in couplings with the Higgs. 
\begin{align}
 \mathcal{L}_{H} \equiv& \lambda_d \overline{\widehat{\Psi}^c}\left( -i\sigma_2^{*}  H^{*}\right)^{*} (\widehat{N}^{c})_L
+\lambda_u \overline{\widehat{\Psi}^c}\left( -i\sigma_2^{*}  H^{*}\right)^{*} \widehat{N}_R+\text{h.c} \nonumber\\
=&\lambda_d \overline{\widehat{\Psi}^c}\left( i\sigma_2  H^{*}\right)^{*} (\widehat{N}_R)^c
+\lambda_u \overline{\widehat{\Psi}^c}\left( i\sigma_2  H^{*}\right)^{*} \widehat{N}_R+\text{h.c}\nonumber\\
  =&\lambda_d \overline{\widehat{\Psi}^c} \widetilde{H}^{*} (\widehat{N}_R)^c
+\lambda_u \overline{\widehat{\Psi}^c}\widetilde{H}^{*}  \widehat{N}_R+\text{h.c}\,.
\end{align}
Taking into account that
\begin{align*}
  \overline{\widehat{\Psi}^c} \widetilde{H}^{*} (\widehat{N}_{R})^{c}=&\overline{\left[ (\widehat{N}_R)^c \right]^c} \left( \widetilde{H}^{*}  \right)^{\operatorname{T}}\left( \widehat{\Psi}^c \right)^c \nonumber\\
  \overline{\widehat{\Psi}^c} \widetilde{H}^{*} (\widehat{N}_{R})=&\overline{ (\widehat{N}_R)^c } \left( \widetilde{H}^{*}  \right)^{\operatorname{T}}\left( \widehat{\Psi}^c \right)^c \,,
\end{align*}
we have
\begin{align*}
    \mathcal{L}_H=&\lambda_d \overline{\widehat{N}_R} \left( \widetilde{H}^{*} \right)^{\operatorname{T}} \widehat{\Psi}
+\lambda_u \overline{(\widehat{N}_R)^c}\left( \widetilde{H}^{*} \right)^{\operatorname{T}}  \widehat{\Psi}+\text{h.c}\nonumber\\
  =&\lambda_d \overline{\widehat{N}_R} \widetilde{H}^{\dagger} \widehat{\Psi}
+\lambda_u \overline{(\widehat{N}_R)^c}\widetilde{H}^{\dagger} \widehat{\Psi}+\text{h.c}  \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}} \widetilde{H}\widehat{N}_R
+\lambda_u \overline{\widehat{\Psi}} \widetilde{H} (\widehat{N}_R)^{c}+\text{h.c}  \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}} \widetilde{H}\widehat{N}_R
+\lambda_u \overline{\widehat{\Psi}} \widetilde{H} (\widehat{N}^c)_L+\text{h.c}  \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}} \widetilde{H}P_R\widehat{N}
+\lambda_u \overline{\widehat{\Psi}} \widetilde{H} P_L\widehat{N}^{c}+\text{h.c} \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}_L} \widetilde{H}\widehat{N}
+\lambda_u \overline{\widehat{\Psi}_R} \widetilde{H} \widehat{N}^{c}+\text{h.c}
\end{align*}

From eq.~\eqref{eq:NM} 
\begin{align}
  \widehat{N}^{c}=&
\begin{pmatrix}
  \left( N^{\dagger} \right)^{\dagger} \\ 
  N^{\dagger} 
\end{pmatrix}+
\begin{pmatrix}
  N \\ 
  N^{\dagger} 
\end{pmatrix}=\widehat{N}
\end{align}
and we have
\begin{align}
    \mathcal{L}_A=&M_D \overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}
+h_{i\alpha} \overline{\widehat{\Psi}_{R}} \widehat{L}_i S_{\alpha}
+ \lambda_d \overline{\widehat{\Psi}_L}\widetilde{H} \widehat{N}
+\lambda_u \overline{\widehat{\Psi}_{R}}\widetilde{H}\widehat{N}+\text{h.c}\,,
\end{align}
as expected from eq.~\eqref{eq:lfull}
}
%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsNeutralWyelLagrangian}{
\begin{align}
  \mathcal{L}_0=&h_{i\alpha}N_{3n}\chi_n \nu_{Li}S_\alpha+\frac{1}{2}\mathbf{X}^{\operatorname{T}}\mathbf{N}^{\dagger} \mathbf{M}^{\chi}\mathbf{N}\mathbf{X}+\text{h.c}\nonumber\\
=&h_{i\alpha}N_{3n}\chi_n \nu_{Li}S_\alpha+\frac{1}{2}\chi_{m}\left( \mathbf{M}^{\chi}_{\text{diag}} \right)_{mn} \chi_{n} +\text{h.c}
\end{align}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsNeutrinoMassInteractionBasis}{
The result from \cite{Bonnet:2012kz} when  adapted to our case, imply that ($\lambda_d \to Y_L\; \lambda_u \to Y_R$)


%check nuint.pdf
\begin{align}
 -i\dfrac{ M^{\nu}_{ij}}{v^2}=2\sum_{\alpha}h_{i\alpha}h_{j\alpha} &\left[  \lambda_u^2\int \frac{d^4 k}{(2\pi)^4}i S_F \left(k,M_D \right)P_R i S_F \left(k,M_N \right)P_R i S_F \left(k,M_D \right)
             i \Delta_F \left( k+p,m_{S_\alpha} \right)\right. \nonumber\\
          &\left.+\lambda_d^2\int \frac{d^4 k}{(2\pi)^4}i S_F \left(k,M_D \right)P_L i S_F \left(k,M_N \right)P_L i S_F \left(k,M_D \right)
            i \Delta_F \left( k+p,m_{S_\alpha} \right) 
            \right].
\end{align}

\begin{align}
  M^{\nu}_{ij}=&-\sum_{\alpha}\frac{2h_{i\alpha}h_{j\alpha}v^2 M_N}{(4\pi)^2} 
      \left[\lambda_u^{2} \, J_4\left(M_D^2,M_D^2,M_N^2,m^{2}_{S_\alpha}  \right)
            + \lambda_d^2 M_D^2  \, I_4\left(M_D^2,M_D^2,M_N^2,m^2_{S_\alpha}  \right)
      \right]\nonumber\\
=&-\sum_{\alpha}\frac{2h_{i\alpha}h_{j\alpha}v^2 M_N \lambda^2 \cos^2\beta}{(4\pi)^2} 
      \left[\tan^2\beta \, J_4\left(M_D^2,M_D^2,M_N^2,m^{2}_{S_\alpha}  \right)
            +  M_D^2  \, I_4\left(M_D^2,M_D^2,M_N^2,m^2_{S_\alpha}  \right)
      \right]\nonumber\\
\end{align}
where
\begin{align}
   J_4\left(M_D^2,M_D^2,M_N^2,m^2_{S_\alpha}  \right)=&\frac{(4\pi)^2}{i}
   \int \frac{d^4 k}{(2\pi)^4}
\frac{k^2}{\left(k^2-m_D^2\right)^2\left( k^2-M_N^2 \right)\left(k^2-m_{S_\alpha}^2\right)} \nonumber\\
   I_4\left(M_D^2,M_D^2,M_N^2,m^2_{S_\alpha}  \right)=&\frac{(4\pi)^2}{i}
   \int \frac{d^4 k}{(2\pi)^4}
\frac{1}{\left(k^2-m_D^2\right)^2\left( k^2-M_N^2 \right)\left(k^2-m_{S_\alpha}^2\right)}.
\end{align}
After integration
%see calculoij.pdf
\begin{align*}
  J_4\left(M_D^2,M_D^2,M_N^2,m^2_{S_\alpha}  \right)=
-&\left\{  \left[\frac{M_D^2}{\left(M_N^2-M_D^2\right)\left(m_{S_\alpha}^2-M_D^2\right)} 
-\frac{M_D^4 \left(2M_D^2-M_N^2-m_{S_\alpha}^2\right)}{2\left(M_N^2-M_D^2\right)^2\left(m_{S_\alpha}^2-M_D^2\right)^2} \right]\ln M_D^2\right.\nonumber\\
&-\frac{M_N^4\ln M_N^2}{2\left( m_{S_\alpha}^2-M_N^2 \right)\left( M_D^2-M_N^2 \right)^2}-
\frac{m_{S_\alpha}^4\ln m_{S_\alpha}^2}{2\left( m_N^2-m_{S_\alpha}^2 \right)\left( M_D^2-m_{S_\alpha}^2 \right)^2}
\nonumber\\
 &\left.+\frac{M_D^2}{2\left(M_N^2-M_D^2  \right)\left(m_{S_\alpha}^2-M_D^2  \right)} \right\},
\end{align*}
%\begin{align}
%      I_4&\left(M_D^2,M_D^2,M_N^2,m^2_{S}  \right)=\nonumber\\
%&\left[\frac{M_N^2\ln \left( M_N^2/M_D^2 \right)}{\left( M_N^2-M_D^2 \right)^4\left( M_N^2-m_{S_\alpha}^2 \right)^2%}
%      -\frac{m_{S_\alpha}^2\ln \left( m_{S_\alpha}^2/M_D^2 \right)}{\left( m_{S_\alpha}^2-M_D^2 \right)^4\left( M_N%^2-m_{S_\alpha}^2 \right)^2}-
%      \frac{1}{\left(m_{S_\alpha}^2-M_D^2\right)^2\left(M_N^2 -M_D^2 \right)^2} 
% \right],
%\end{align}
%or
\begin{align}
   I_4\left(M_D^2,M_D^2,M_N^2,m^2_{S_\alpha}  \right)=
&\left[ \frac{\left(M_D^4-M_N^2 m_{S_\alpha}^2\right)\ln M_D^2}{\left(M_N^2 -M_D^2 \right)^2\left(m_{S_\alpha}^2 -M_D^2 \right)^2} 
+\frac{M_N^2 \ln M_N^2}{\left(m_{S_\alpha}^2 -M_N^2 \right)\left(M_D^2-M_N^2\right)^2}\right. \nonumber\\
&\left.+\frac{m_{S_\alpha}^2 \ln m_{S_\alpha}^2}{\left(M_N^2 -m_{S_\alpha}^2 \right)\left(M_D^2-m_{S_\alpha}^2\right)^2} 
-\frac{1}{\left(m_{S_\alpha}^2-M_D^2\right)\left(M_N^2 -M_D^2 \right)} 
\right].
\end{align}



In  \cite{Fraser:2014yha} only the contribution proportional to $\lambda_u$ is considered in the limit $M_N\to 0$\footnote{$\lim_{x\to 0}x\ln x=\lim_{x\to 0}\dfrac{\ln x}{1/x}=0$}, 
\begin{align*}
   J_4\left(M_D^2,M_D^2,M_N^2,m^2_{S}  \right)=&
-\left\{  \left[-\frac{M_D^2}{M_D^2\left(m_{S}^2-M_D^2\right)} 
-\frac{M_D^4 \left(2M_D^2-m_{S_\alpha}^2\right)}{2M_D^4\left(m_{S}^2-M_D^2\right)^2} \right]\ln M_D^2\right.\nonumber\\
&\qquad+\frac{m_{S_\alpha}^4\ln m_{S_\alpha}^2}{2m_{S_\alpha}^2\left( M_D^2-m_{S_\alpha}^2 \right)^2} 
\left.-\frac{M_D^2}{2M_D^2\left(m_{S_\alpha}^2-M_D^2  \right)} \right\}\nonumber\\
=&  -\left\{  -\left[\frac{1}{\left(m_{S}^2-M_D^2\right)} 
+\frac{\left(2M_D^2-m_{S_\alpha}^2\right)}{2\left(m_{S}^2-M_D^2\right)^2} \right]\ln M_D^2
+\frac{m_{S_\alpha}^2\ln m_{S_\alpha}^2}{2\left( M_D^2-m_{S_\alpha}^2 \right)^2} 
-\frac{1}{2\left(m_{S_\alpha}^2-M_D^2  \right)} \right\}\nonumber\\
=&  -\frac{1}{\left(m_{S}^2-M_D^2\right)}\left\{  -\left[1 
+\frac{\left(2M_D^2-m_{S_\alpha}^2\right)}{2\left(m_{S}^2-M_D^2\right)} \right]\ln M_D^2
+\frac{m_{S_\alpha}^2\ln m_{S_\alpha}^2}{2\left( M_D^2-m_{S_\alpha}^2 \right)} 
-\frac{1}{2} \right\}\nonumber\\
= & \frac{1}{2\left(m_{S}^2-M_D^2\right)}\left\{  \frac{m_{S_\alpha}^2\ln M_D^2}{\left(m_{S}^2-M_D^2\right)}
-\frac{m_{S_\alpha}^2\ln m_{S_\alpha}^2}{\left( M_D^2-m_{S_\alpha}^2 \right)} +1 \right\}\nonumber\\
=&  \frac{1}{2\left(m_{S}^2-M_D^2\right)}\left[ 1+ \frac{m_{S_\alpha}^2\ln \left( M_D^2/m_{S_\alpha}^2 \right)}{\left(m_{S}^2-M_D^2\right)}
\right]\nonumber\\
=& - \frac{1}{2\left(M_D^2-m_{S}^2\right)}\left[ 1-\frac{m_{S_\alpha}^2\ln \left( M_D^2/m_{S_\alpha}^2 \right)}{\left(M_D^2-m_{S}^2\right)}
\right].
\end{align*}
So that
\begin{align*}
M^{\nu}_{ij}=\sum_{\alpha}\frac{h_{i\alpha}h_{j\alpha}\left(\lambda_u^2 v^2\right)M_N}{16\pi^2\left(M_D^2-m_{S_\alpha}^2\right)}
\left[ 1-\frac{m_{S_\alpha}^2\ln \left( M_D^2/m_{S_\alpha}^2 \right)}{\left(M_D^2-m_{S_\alpha}^2\right)}\right].
\end{align*}
}

%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsNeutrinoMassEigenBasis}{  
In order to compute the neutrino mass matrix we need to remenbert that the correction to one fermionic propagator is given by $S_F^{-1}=(\slashed{p}-m)-\Sigma(p)$. We use the Feynman rules in order to compute the $\Sigma$ amplitud (neutrino propagator correction).
\begin{align*}
  -i\Sigma^{\nu}_{ij}(p)=&\sum_{\alpha}\int \frac{d^4k}{(2\pi)^4}\sum_{n=1}^3 \left( i h_{i\alpha} N_{3n} \right) i S_F(k)\left( i h_{j\alpha} N_{3n} \right)i\Delta_F(p+k)\nonumber\\
=&i\sum_{\alpha}\frac{h_{i\alpha}h_{j\alpha}}{16\pi^2}\sum_{n=1}^3 \left( N_{3n} \right)^2\int \frac{d^4k}{i\pi^2}\frac{\cancel{k}+m_{\chi_n}}{\left(k^2-m_{\chi_n}^2  \right)\left[\left(p+k\right)^2-m_{S_\alpha}^2\right]}
\end{align*}

therefore

\begin{align*}
  -iM^{\nu}_{ij}(p)=&i\sum_{\alpha}\frac{h_{i\alpha}h_{j\alpha}}{16\pi^2}\sum_{n=1}^3 \left( N_{3n} \right)^2\int \frac{d^4k}{i\pi^2}\frac{\cancel{k}+m_{\chi_n}}{\left(k^2-m_{\chi_n}^2  \right)\left[\left(p+k\right)^2-m_{S_\alpha}^2\right]}
\end{align*}

Therefore in the limit $p\to 0$, we have
}
%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsPassarinoVeltman}{
  
\begin{align*}
  B_0 \left(0;m_{\chi_n}^2,m^2_{S_{\alpha}} \right)=&\int \frac{d^4k}{i\pi^2}\frac{1}{\left(k^2-m_{\chi_n}^2\right)\left(k^2-m_{S_\alpha}^2\right)}\nonumber\\
            =&\frac{1}{m_{\chi_n}^2-m_{S_\alpha}^2}\left[ A_0\left(m_{\chi_n}^2\right)-A_0\left(m_{S_\alpha}^2\right)  \right],
\end{align*}
and
\begin{align*}
  A_0\left(m^2\right)=m^2 \left[ \Delta+1-\ln \left( m^2/\mu^2 \right) \right]
\end{align*}
with
\begin{align*}
  \Delta=\left( \frac{2}{\epsilon}-\ln\pi+\gamma_E \right),
\end{align*}
where $\mu$ is the subtraction point (dimensional regularization) an $\gamma_E$ is the Euler-Mascheroni constant.
Replacing back in eq.~\eqref{eq:mnueig}, we have
\begin{align}
\label{eq:mnueigdev}
\sum_{n=1}^3& \left( N_{3n} \right)^2m_{\chi_n}\; B_0 \left(0;m_{\chi_n}^2,m^2_{S_\alpha} \right)\nonumber\\
  &=\sum_{n=1}^3 \left( N_{3n} \right)^2m_{\chi_n}
   \left\{\frac{1}{m_{\chi_n}^2-m_{S_\alpha}^2}\left[m^2_{\chi_n} \left[ \Delta+1-\ln \left( m_{\chi_n}^2/\mu^2 \right) \right]  \right] 
-m_{S_\alpha}^2 \left[ \Delta+1-\ln \left( m_{S_\alpha}^2/\mu^2 \right) \right] \right\}\nonumber\\
&=\sum_{n=1}^3 \left( N_{3n} \right)^2m_{\chi_n}
   \left\{(\Delta+1)+\frac{m_{S_\alpha}^2\ln \left( m_{S_\alpha}^2/\mu^2 \right)-m_{\chi_n}^2\ln \left( m_{\chi_n}^2/\mu^2 \right)}{m_{\chi_n}^2-m_{S_\alpha}^2} \right\}\nonumber\\
&=\sum_{n=1}^3 \left( N_{3n} \right)^2m_{\chi_n}
   \left\{\left[\Delta+1+\ln\left( \mu^2 \right) \right]+\frac{m_{S_\alpha}^2\ln \left( m_{S_\alpha}^2 \right)-m_{\chi_n}^2\ln \left( m_{\chi_n}^2 \right)}{m_{\chi_n}^2-m_{S_\alpha}^2} \right\}\,.
\end{align}

From equation \ref{eq:chidiag} we have that 
\begin{align*}
  \mathbf{N} \mathbf{M}^\chi_{\text{diag}}\mathbf{N}^{\operatorname{T}}=\mathbf{M}^\chi\Rightarrow \sum_mN_{lm}m_{\chi_m} N_{nm}=(\mathbf{M}^\chi)_{ln}.
\end{align*}
}
%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsMutoEGamma}{
\subsubsection{$\mu  \rightarrow e \gamma$ decay}
A loop computation of $\mu  \rightarrow e \gamma$ into our model has account of the coupling to the photon with the new charge fermions and the coupling into the SM leptons, the new charge fermions and the new  neutral scalars.
The three diagrams important for this computations are: (diagrams)\\
 
According with \cite{Lavoura:2003xp} for the radiative decay $f_1(p_1)  \rightarrow f_2(p_2) \gamma (q)$ where $q=p_1-p_2$, $f_1$ has a mass $m_1$ and $f_2 $ has a mass $m_2$ we can calculate the process if we know the Yukawa lagrangian.
We take the fermions on shell: $p_1=m_1^2$  y $p_2=m_2^2$. They are represented by spinors $u_1$ and $u_2$, which satisfy $\cancel{p}_1u_1=m_1u_1$ and $\bar{u}_2\cancel{p}_2=m_2\bar{u}_2$.

The amplitude for the decay is $\epsilon^*_{\mu}(q)M^{\mu}$, where $\epsilon^*_{\mu}$ is the outgoing photon polarization and $e$ is the electric charge of the positron. We know that the gauge invariance implies that $q_{\mu}M^{\mu}$ must be zero, therefore according with \cite{Lavoura:2003xp} the $M^{\mu}$ has the form:
\begin{align}
M^{\mu}=\bar{u}_2(p_2)( \sigma_L\Sigma_L^{\mu}+\sigma_R\Sigma_R^{\mu} +O^{\mu} )u_1(p_1)
\end{align}
Where:
\begin{align}
\Sigma_L^{\mu}=&(p_1^{\mu}+p_2^{\mu})P_L-\gamma^{\mu}(m_2P_L+m_1P_R)\\	
\Sigma_R^{\mu}=&(p_1^{\mu}+p_2^{\mu})P_R-\gamma^{\mu}(m_2P_R+m_1P_L)
\end{align}

We only take care of $\sigma_{L}$ and $\sigma_{R}$ factors, not for $O^{\mu}$, because they are the only relevant parameters important for $f_1 \rightarrow f_2 \gamma$ decay and on-shell photon. Therefore we will not put the $O^{\mu}$ term anymore.

Alternatively we can write $M^{\mu}$ in the form:
\begin{align}
M^{\mu}=\bar{u}_2(p_2)( i\sigma^{\mu\nu}q_{\nu}(\sigma_LP_L+\sigma_RP_R))u_1(p_1)
\end{align}

In general the partial width for $f_1\rightarrow f_2\gamma$ is given by:

\begin{align}
\boxed{\Gamma = \dfrac{(m_1^2-m_2^2)^3(|\sigma_L|^2+|\sigma_R|^2)}{16\pi m_1^3}}
\label{partial_width_muegamma}
\end{align}

With all this in mind, our work is determinate the $\sigma_L$ and the $\sigma_R$ in T13A model and use the eq. (\ref{partial_width_muegamma}).

\subsubsection{$\sigma_L$ and $\sigma_R$ in T13A}

In general for a Yukawa interaction to the form:
\begin{align}
\mathcal{L}_{\text{Yukawa}}=B\overline{F}(L_iP_L+R_iP_R)f_i+B^*\overline{f}_i(L_i^*P_R+R_i^*P_L)F
\end{align}
Where the fermions $f_i$ have charge $Q_f=e$ and the spin$-0$ boson $B$ have charge $Q_B$ and the fermions $f_i$ have interaction with the boson $B$ and spin$-1/2$ fermion $F$ with arbitrary dimensionless numerical coefitients $L_1,L_2$, $R_1$ and $R_2$, the $\sigma_L$ and $\sigma_R$ are:
\begin{align}
\sigma_L=& Q_f(\rho k_1 +\lambda k_2 + v k_3)+Q_B(\rho \overline{k}_1 + \lambda \overline{k}_2 + v \overline{k}_3)\\
\sigma_R=& Q_f(\lambda k_1 +\rho k_2 + \zeta k_3)+Q_B(\lambda \overline{k}_1 + \rho \overline{k}_2 + \zeta \overline{k}_3)
\end{align} 
with:
\begin{align}
\lambda=&L_2^*L_1\\
\rho=&R_2^*R_1\\
\zeta=&L_2^*R_1\\
v=&R_2^*L_1\\
k_1=&m_1(c_1+d_1+f)\\
k_2=&m_2(c_2+d_2+f)\\
k_3=&m_F(c_1+c_2)
\end{align}
the other are not important because in T13A $Q_B=0$.

In the T13A($\alpha=0$) model we have the next term in the Yukawa lagrangian:
\begin{align}
\mathcal{L}&\supset h_{i\alpha}\overline{e_{Li}}\psi^-_{R}S_\alpha+ h.c\\
&=S_\alpha\overline{\psi^-}[h_{i\alpha}P_L]e_i + S_\alpha\overline{e_i}[h_{i\alpha}P_R]\psi^- 
\end{align}
therefore we can do the next identification:
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
B $\rightarrow S_\alpha$ & $R_i \rightarrow  0$ & $R_i^* \rightarrow  h_{i\alpha}$  \\
F $\rightarrow \psi^-$ & $L_i \rightarrow h_{i\alpha}$ & $L_i^* \rightarrow  0$ \\
$f_i \rightarrow e_{i}$ &  & \\ 
\hline
\end{tabular}
\end{center}
and we have:
\begin{align}
\sigma_L=&eh_{2\alpha}h_{1\alpha}m_1(c_1+d_1+f)=eh_{2\alpha}h_{1\alpha}m_1(c_1+\dfrac{3}{2}d) \nonumber \\
\sigma_R=&eh_{2\alpha}h_{1\alpha}m_2(c_2+d_2+f)=eh_{2\alpha}h_{1\alpha}m_2(c_2+\dfrac{3}{2}d) \approx 0
\label{sigmas}
\end{align}
In the last equation I used the relation $d_1=d_2=2f=d$ and $m_1=m_{\mu} \gg m_2=m_{e}$.

According with \cite{Lavoura:2003xp}, the parameter $c_i=c,d_i=d$ and $f$ are related with the loop integrals. Particularly we have:
\begin{align}
\bigg(c+\dfrac{3}{2}d\bigg)=&\dfrac{i}{16\pi^2 m_B^2}\bigg[\dfrac{x^2-5x-2}{12(x-1)^3}+\dfrac{x \ln x}{2(x-1)^4}\bigg]=\dfrac{i}{16\pi^2 m_B^2} \boxed{\dfrac{1}{2}}\bigg[\dfrac{x^3-6x^2+3x+2+6x\ln x}{6(x-1)^4}\bigg]
\end{align}
where $x=\dfrac{m_F^2}{m_{\phi}^2}$. 

Finally putting all this in the eq. (\ref{sigmas}) we have:
\begin{align}
\sigma_L=&\dfrac{i eh_{2\alpha}h_{1\alpha}m_{\mu}}{16\pi^2 m_B^2}\dfrac{1}{2}F(x)\nonumber \\
\sigma_R \approx & 0
\label{sigmas_result}
\end{align}
where: 
\begin{align}
F(x)=\bigg[\dfrac{x^3-6x^2+3x+2+6x\ln x}{6(x-1)^4}\bigg] \hspace{1 cm} \text{with} \hspace{1 cm} x=\dfrac{M_D^2}{m_{S_{\alpha}}^2}
\label{Fx}
\end{align}

\subsubsection{Branching( $\mu \rightarrow e \gamma$ )}
Putting the eq.(\ref{sigmas_result}) into the eq.(\ref{partial_width_muegamma}) we have:
\begin{align}
\Gamma(\mu \rightarrow e \gamma) =&\frac{(m_{\mu}^2-m_e^2)^3}{16\pi m_{\mu}^3}(|\sigma_L|^2) \approx \frac{m_{\mu}^3 |\sigma_L|^2}{16\pi}\nonumber \\
=& \frac{m_{\mu}^5}{16\pi}\bigg| \frac{e h_{1\alpha}h_{2\alpha}}{16 \pi^2 m_{S_\alpha}^2} \frac{F(x)}{2} \bigg|^2
\end{align}
therefore:
\begin{align}
  Br(\mu \rightarrow e \gamma) =& \frac{\Gamma(\mu \rightarrow e \gamma )}{\Gamma(\mu \rightarrow e \bar{\nu}_e \nu_{\mu})}=\frac{\frac{m_{\mu}^5}{16\pi}\bigg| \frac{e h_{1\alpha}h_{2\alpha}}{16 \pi^2 m_{S_\alpha}^2} \frac{F(x)}{2} \bigg|^2}{ \frac{G_F^2 m_{\mu}^5}{192\pi^3} } \nonumber \\
=&\frac{3}{4}\frac{1}{G_F^2}\bigg(\frac{e^2}{4\pi}\bigg)\frac{1}{16\pi}\bigg|\frac{F(x)h_{1\alpha}h_{2\alpha}}{m_{S_\alpha}^2}\bigg|^2 
\end{align}
}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\DetailsAnalyticformulas}{

\section{Analytic formulas for the masses and the mixing parameters of the $\chi_n$ neutral fermions}

\subsection{Fermionic neutral masses}

The neutral masses are determinated from the eigenvalue equation: $\text{Det}(\mathbf{M}^{\chi}-(\mathbf{M}^{\chi}_{diag})_{ii})=0$.
Using the eq. \ref{eq:Mchi} we get:
\begin{equation}
((\mathbf{M}^{\chi}_{diag})_{ii})^3-M_N((\mathbf{M}^{\chi}_{diag})_{ii})^2-(M_D^2+\lambda^2 \dfrac{v^2}{2})(\mathbf{M}^{\chi}_{diag})_{ii}+(M_NM_D^2-2\lambda^2\sin\beta\cos\beta M_D)=0 \nonumber
\end{equation}
In order to have a more compact notation we will call $(\mathbf{M}^{\chi}_{diag})_{ii})$ like $m_i$, and therefore we have to solve the next equation:
\begin{equation}
m_i^3-M_Nm_i^2-(M_D^2+\lambda^2 \dfrac{v^2}{2})m_i+(M_NM_D^2-2\lambda^2\sin\beta\cos\beta M_D)=0 
\end{equation}

The solutions to this equation are:

\begin{eqnarray}
m_1=z_2+\dfrac{M_N}{3} \hspace{1.0 cm}
m_2=z_1+\dfrac{M_N}{3} \hspace{1.0 cm}
m_3=z_3+\dfrac{M_N}{3}
\end{eqnarray}
Where:
\begin{eqnarray}
z_1&=&\bigg(-\dfrac{q}{2}+\sqrt{\dfrac{q^2}{4}+\dfrac{p^3}{27}}\bigg)^{1/3} + \bigg(-\dfrac{q}{2}-\sqrt{\dfrac{q^2}{4}+\dfrac{p^3}{27}}\bigg)^{1/3}\\
z_2&=&-\dfrac{z_1}{2}+\sqrt{\dfrac{z_1^2}{4}+\dfrac{q}{z_1}} \\
z_3&=&-\dfrac{z_1}{2}-\sqrt{\dfrac{z_1^2}{4}+\dfrac{q}{z_1}}\\
p&=&-\dfrac{1}{3}M_N^2-(M_D^2+\lambda^2 \dfrac{v^2}{2}) \hspace{0.7 cm} \\
q&=&-\dfrac{2}{27}M_N^3-\dfrac{1}{3}M_N(M_D^2+\lambda^2 \dfrac{v^2}{2})+(M_NM_D^2-2\lambda^2\sin\beta\cos\beta M_D)
\end{eqnarray}

Notice that $\dfrac{q^2}{4}+\dfrac{p^3}{27} < 0$ and therefore, we have three real masses $m_i$ $(i=1,2,3)$.

To order $\lambda^2$ the fermionic masses are given by:

\begin{eqnarray}
m_1&=&M_N+\dfrac{v^2(M_N+M_D\sin(2\beta))}{2(M_N^2-M_D^2)}\lambda^2 + O(\lambda^4)\\
m_2&=&M_D- ... \\
m_3&=&-M_D- ...
\end{eqnarray}



\subsection{Mixing matrix $\textbf{N}$}
We know that: 
\begin{equation}
\textbf{N}^{\dagger } \textbf{M}^{\chi}\textbf{N}=\textbf{M}^{\chi}_{\text{diag}}=\text{Diag}(m_{i}) \rightarrow \textbf{N}^{\dagger}\textbf{M}^{\chi}-\text{Diag}(m_i)\textbf{N}^{\dagger}=0
\end{equation}

Equating the elements of the ith row of the last equation, we get:
\begin{eqnarray}
[\textbf{M}^{\chi}_{11}-m_i]\textbf{N}_{1i} + \textbf{M}^{\chi}_{21}\textbf{N}_{2i}+\textbf{M}^{\chi}_{31}\textbf{N}_{3i}=0 \\ \nonumber
\textbf{M}^{\chi}_{12}\textbf{N}_{1i}+[\textbf{M}^{\chi}_{22}-m_i]\textbf{N}_{2i}+\textbf{M}^{\chi}_{32}\textbf{N}_{3i}=0 \\ \nonumber
\textbf{M}^{\chi}_{13}\textbf{N}_{1i}+\textbf{M}^{\chi}_{23}\textbf{N}_{2i}+[\textbf{M}^{\chi}_{33}-m_i]\textbf{N}_{3i}=0 
\end{eqnarray}

Dividing the three equation by $\textbf{N}_{1i}$, where it is assumed that $\textbf{N}_{1i}\neq 0$, the system becomes:

\begin{eqnarray}
\textbf{M}^{\chi}_{21}\dfrac{\textbf{N}_{2i}}{\textbf{N}_{1i}}+\textbf{M}^{\chi}_{31}\dfrac{\textbf{N}_{3i}}{\textbf{N}_{1i}}&=&-(\textbf{M}^{\chi}_{11}-m_i) \\
(\textbf{M}^{\chi}_{22}-m_i)\dfrac{\textbf{N}_{2i}}{\textbf{N}_{1i}}+\textbf{M}^{\chi}_{32}\dfrac{\textbf{N}_{3i}}{\textbf{N}_{1i}}&=&-\textbf{M}^{\chi}_{12} \\
\textbf{M}^{\chi}_{23}\dfrac{\textbf{N}_{2i}}{\textbf{N}_{1i}}+(\textbf{M}^{\chi}_{33}-m_i)\dfrac{\textbf{N}_{3i}}{\textbf{N}_{1i}}&=&-\textbf{M}^{\chi}_{13}
\end{eqnarray}

Using the matrix $\textbf{M}^{\chi}$ given in the eq. \ref{eq:Mchi}, we get the ratios

\begin{eqnarray}
\dfrac{\textbf{N}_{2i}}{\textbf{N}_{1i}}&=&\dfrac{v}{\sqrt{2}}\dfrac{\lambda_d}{m_i}-\dfrac{M_D}{m_i}\dfrac{\sqrt{2}}{v}\dfrac{[m_i(M_N-m_i)+\lambda_d^2 v^2/2]}{(\lambda_u m_i+\lambda_d M_D)} \\  \nonumber
&=&\dfrac{v}{\sqrt{2}}\dfrac{\lambda \cos\beta}{m_i}-\dfrac{M_D}{m_i}\dfrac{\sqrt{2}}{v}\dfrac{[m_i(M_N-m_i)+\lambda^2\cos\beta^2 v^2/2]}{\lambda(m_i\sin\beta +M_D\cos\beta )} \\ 
\dfrac{\textbf{N}_{3i}}{\textbf{N}_{1i}}&=&-\dfrac{\sqrt{2}}{v}\dfrac{[m_i(M_N-m_i)+v^2\lambda_d^2/2]}{(\lambda_u m_i+\lambda_dM_D)}\\  \nonumber
&=&-\dfrac{\sqrt{2}}{v}\dfrac{[m_i(M_N-m_i)+v^2\lambda^2 \cos\beta^2/2]}{\lambda_u (m_i\sin\beta+M_D\cos\beta)}
\end{eqnarray}

Finally, recalling the unitary condition on the $\textbf{N}$ matrix we have:

\begin{equation}
\textbf{N}_{1i}^2+\textbf{N}_{2i}^2+\textbf{N}_{3i}^2=1  \nonumber
\end{equation}

for which
\begin{equation}
\textbf{N}_{1i}=\bigg[1+\bigg[\dfrac{\textbf{N}_{2i}}{\textbf{N}_{1i}}\bigg]^2+\bigg[\dfrac{\textbf{N}_{3i}}{\textbf{N}_{1i}}\bigg]^2\bigg]^{-1/2}
\end{equation}

In particular we know that the mixing parameter $\textbf{N}_{3i}$ given in the neutrino mass matrix is given by:
\footnotesize
\begin{eqnarray}
\textbf{N}_{3i}=\dfrac{\bigg(-\dfrac{\sqrt{2}}{v}\dfrac{[m_i(M_N-m_i)+v^2\lambda^2 \cos\beta^2/2]}{\lambda_u (m_i\sin\beta+M_D\cos\beta)}\bigg)}
{\bigg[1+\bigg(-\dfrac{\sqrt{2}}{v}\dfrac{[m_i(M_N-m_i)+v^2\lambda^2 \cos\beta^2/2]}{\lambda_u (m_i\sin\beta+M_D\cos\beta)}\bigg)^2+\bigg(\dfrac{v}{\sqrt{2}}\dfrac{\lambda \cos\beta}{m_i}-\dfrac{M_D}{m_i}\dfrac{\sqrt{2}}{v}\dfrac{[m_i(M_N-m_i)+\lambda^2\cos\beta^2 v^2/2]}{\lambda(m_i\sin\beta +M_D\cos\beta )}\bigg)^2\bigg]^{1/2}}
\end{eqnarray}
\normalsize

To order $\lambda^2$ the $\textbf{N}_{3i}^2$ parameters are given by:

\begin{eqnarray}
\textbf{N}_{31}^2 &=& \dfrac{v^2 (M_D \cos\beta +M_N \sin\beta)^2}{2(M_D^2-M_N^2)^2}\lambda^2 +O(\lambda^4)\\
\textbf{N}_{32}^2 &=& ... +O(\lambda^4)\\
\textbf{N}_{33}^2 &=& ... +O(\lambda^4)
\end{eqnarray}


}
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "t13a"
%%% ispell-local-dictionary: "american"
%%% End:
